The Effectiveness of Memory Replay in Large Scale Continual Learning

We study continual learning in the large scale setting where tasks in the input sequence are not limited to classification, and the outputs can be of high dimension. Among multiple state-of-the-art methods, we found vanilla experience replay (ER) still very competitive in terms of both performance and scalability, despite its simplicity. However, a degraded performance is observed for ER with small memory. A further visualization of the feature space reveals that the intermediate representation undergoes a distributional drift. While existing methods usually replay only the input-output pairs, we hypothesize that their regularization effect is inadequate for complex deep models and diverse tasks with small replay buffer size. Following this observation, we propose to replay the activation of the intermediate layers in addition to the input-output pairs. Considering that saving raw activation maps can dramatically increase memory and compute cost, we propose the Compressed Activation Replay technique, where compressed representations of layer activation are saved to the replay buffer. We show that this approach can achieve superior regularization effect while adding negligible memory overhead to replay method. Experiments on both the large-scale Taskonomy benchmark with a diverse set of tasks and standard common datasets (Split-CIFAR and Split-miniImageNet) demonstrate the effectiveness of the proposed method.

==> compressed activation replay ICLR 2021/experiments.tex <==
\vspace{-2mm}
\section{Preliminaries}
\vspace{-2mm}
In this section, we introduce the problem formulation and evaluation metrics of the type of continual learning problems considered in this work, together with a review of the memory replay basics.

\textbf{Continual learning.} In continual learning, we aim to solve a sequence of supervised learning tasks $(\cT^1, \cT^2, \hdots \cT^t)$, where, $\cT^{i} = \{ (\bx^i_j, \by^i_j) \}_{j=1}^{N_i}$ denotes the data examples for task $i$.  The objective is to perform sequential training while preserving the performance on the past tasks without access to all of their data.
%
Let $\ell^{i}(\cdot, \cdot)$ denote the loss function for task $\cT^i$, which can be any generic loss function (\textit{e.g.,} mean-squared-error or cross entropy), and is not tied to any specific task such as classification. In this work, we adopt an encode-decode model. More specifically, let $g(\cdot)$ denote the shared encoder model, and $h^{i}(\cdot)$ the task head for the task $\cT^i$. Predictions on the task $\cT^i$ are made using the model $p^{i}(\bx) = h^{i}(g(\bx))$. The task loss for optimizing  task $\cT^i$ is then given by
\begin{align}
    \cL^{i}_{task} = \EE_{(\bx, \by) \in \cT^i}~~ \ell^{i}(p^{i}(\bx), \by).
\end{align}

\textbf{Memory replay.} In the simplest version of memory replay based continual learning, we maintain a replay buffer $\cM$ of size $m$ per task (total buffer size is $mt$) for storing samples from the task sequence seen thus far. In addition to task loss, models are optimized using a replay loss given by
\begin{align}
    \cL^{j}_{replay} = \EE_{(\bx_{r}^{j}, \by_{r}^{j}) \in \cM}~~ \ell^{j}(p^{j}(\bx_{r}^{j}), \by_{r}^{j}).
\end{align}
Here, $(\bx_{r}^{j}, \by_{r}^{j})$ denotes the samples from the replay buffer belonging to task $j$. In this work, the data in the replay buffer are sampled uniformly at random from the training data for each task. The overall optimization objective in vanilla experience replay (ER) for training task $i$ is then given by
\begin{align}\label{eq:vanilla_er}
    \min_{g, h^i}~~ \cL^{i}_{task} + \frac{\lambda}{i-1} \sum_{j=1}^{i-1} \cL^{j}_{replay},
\end{align}
where, $\lambda$ is a hyper-parameter that balances the current task loss and the replay losses.

\textbf{Evaluation metric.}
One of the challenges in continual learning with non-classification tasks (textit{e.g.,}, Taskonomy dataset) is the evaluation metric. In this work, for Taskonomy, we propose \emph{forgetting} and \emph{performance drop} as two major metrics. Let $\ell_{test}(i, j)$ denote the test loss of task $j$ using the model snapshot obtained at the end of training task $i$ in the task sequence, and let $\ell^{MT}_{test}(i)$ denote the test loss of task $i$ obtained from a multi-task model trained simultaneously on all tasks. Then, the two metrics are defined as follows:
\begin{align*}
    \text{Forgetting :=}&~~~~ \frac{1}{t}\sum_{i=1}^{t} \frac{\ell_{test}(t, i) - \ell_{test}(i, i)}{\ell_{test}(i, i)} \times 100\%     \\
    \text{Performance drop :=}&~~~~ \frac{1}{t}\sum_{i=1}^{t} \frac{\ell_{test}(t, i) - \ell^{MT}_{test}(i)}{\ell^{MT}_{test}(i)} \times 100\%
\end{align*}
The \emph{forgetting} measure indicates the average loss increase of the model compared to the model snapshot at the end of $i^{th}$ task, while the \emph{performance drop} quantifies the performance drop of the final model compared to a multi-task model trained using the same model architecture.

For classification tasks, \textit{e.g.,} Split-CIFAR and Split-miniImageNet, we report \emph{forgetting} and \emph{average accuracy} as two main metrics. Specifically, let $Acc(i, j)$ denotes the accuracy on task $j$ using the model snapshot obtained at the end of training task $i$. We have
\begin{align*}
   \text{Forgetting :=}~~~~ \frac{1}{t}\sum_{i=1}^{t} \max_{j} \left[ Acc(j, i) - Acc(t, i) \right], \quad \text{Avg accuracy :=}~~~~ \frac{1}{t}\sum_{i=1}^{t} Acc(t, i).
\end{align*}


\section{Vanilla experience replay is a strong baseline}\label{sec:vanilla_er}

We begin our study by investigating the performance of different classes of continual learning algorithms on Taskonomy, which is a large scale dataset with diverse set of tasks. We compare to Side-Tuning~\citep{sidetuning2020}, an expansion based method mentioned in Section~\ref{sec:related_work}, EWC~\citep{Kirkpatrick_2017}, a regularization algorithm that constructs the regularizer based on the Fisher information of the model's weights, A-GEM~\citep{chaudhry2018efficient} a memory replay baseline that uses replay examples to construct a constrained optimization problem, and finaly ER the vanilla experience replay algorithm described in~\eqref{eq:vanilla_er}. For completeness, we also compare with the vanilla SGD algorithm that trains the model sequentially on all the tasks without storing extra information, and the multi-task (MT) algorithm which has access to all the tasks simultaneously.

%based on taskonomy dataset. We perform experiments using several state-of-the-art methods on the Taskonomy benchmark. 



\subsection{Experiment setup}

Taskonomy \citep{zamir2018taskonomy} is a large scale dataset of indoor scenes from various buildings containing annotations for several diverse computer vision tasks. We use data from the following $11$ tasks in this work: \textit{curvature estimation, object classification, scene classification, surface normal estimation, semantic segmentation, depth estimation, reshading, edge detection (texture), edge detection (occlusion), 2D keypoint estimation and 3D keypoint estimation}. All input samples are of $256 \times 256$ resolution. We use a subset of Taskonomy dataset containing $50$ buildings in all our experiments. Of these, $5$ randomly chosen buildings are treated as held-out test set, while the rest of the data are used for training and validation. This yields a total training size of $324,864$ samples.

\textbf{Loss function.} Following \cite{zamir2018taskonomy}, object and scene classification tasks are trained using cross entropy loss, semantic segmentation using pixelwise cross entropy, curvature estimation using $\ell_1$ loss, and all other tasks using $\ell_2$ loss.

\textbf{Model.} We use Resnet-50 model as our encoder network $g(\cdot)$. Since most tasks in Taskonomy dataset are pixel-wise tasks, we do not perform the spatial average pooling in the pen-ultimate layer of Resnet-50 model. This results in a feature map of dimension $2048 \times 8 \times 8$. Following \cite{zamir2018taskonomy}, we use $15$-layer ConvNet model with upsampling blocks as the task heads $h^i$.

\begin{table*}
\caption{\small\textbf{Taskonomy results} using various methods. Forgetting and performance drop ($\Delta$Performance) values are reported. $11$ different tasks are used. All results are averaged over $3$ random seeds. ER-$m$ means we store $m$ data examples for each task. Top two results for forgetting and performance are highlighted in \textbf{bold}. }\vskip -1em
\label{tab:taskonomy_1}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r | cccc  ccc}
\toprule
Method & MT & SGD & Side-Tuning & EWC & A-GEM & ER-64 & ER-256\\
& - & - & (expansion) & (regularization) & (replay) & (replay) & (replay)\\
\midrule
Extra Storage (GB) & 410\footnotemark & 0 & 0.46 & 5.40\footnotemark & 0.44 & 0.11 & 0.44\\
Final model size (GB) & 1.30 & 1.30 & 1.76 & 1.30 & 1.30 &  1.30 &  1.30 \\
Forgetting (\%)& N/A & 191.61 & \bf 0 & 169.62 & 38.88 & 40.18 & \bf 14.73\\
$\Delta$Performance (\%)& \bf 0 & 101.56 & 13.12 & 96.75 & 49.01 & 20.70 & \bf 8.52\\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{center}
\end{table*}

\iffalse
\begin{table*}
\caption{\small\textbf{Taskonomy results} using various methods. Forgetting and performance drop ($\Delta$Performance) values are reported. $11$ different tasks are used. All results are averaged over $3$ random seeds. ER-$m$ means we store $m$ data examples for each task. Top two results for forgetting and performance are highlighted in \textbf{bold}. }\vskip -1em
\label{tab:taskonomy_1}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r | cccc  ccc}
\toprule
Method & MT & SGD & Side-Tuning & EWC & A-GEM & ER-64 & ER-256\\
& - & - & (expansion) & (regularization) & (replay) & (replay) & (replay)\\
\midrule
Extra Storage (GB) & 410\footnotemark & 0 & 0.46 & 5.40\footnotemark & 0.44 & 0.11 & 0.44\\
Final model size (GB) & 1.30 & 1.30 & 1.76 & 1.30 & 1.30 &  1.30 &  1.30 \\
Forgetting (\%)& N/A & 191.61 & \bf 0 & 169.62\std{16.65} & 38.88 & 40.18 & \bf 14.73\std{3.1}\\
$\Delta$Performance (\%)& \bf 0 & 101.56 & 13.12\std{3.84} & 96.75\std{16.46} & 49.01 & 20.70 & \bf 8.52\std{0.5}\\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{center}
\end{table*}
\fi

\subsection{Results}
%\dong{Add discussion here. Saying that ER is better than other algorithms from various aspects, etc. In particular, we should carefully discuss side-tuning.}
Table~\ref{tab:taskonomy_1} contains the result of our large scale analysis. Interestingly, we found that despite its simplicity, the vanilla experience replay algorithm is a strong baseline on Taskonomy. Similar findings were also reported by~\cite{chaudhry2019tiny} but on conventional and mainstream CL datasets like split CIFAR, mini-ImageNet, and CUB which are less realistic, less diverse and smaller in the scale. 
We believe these results indicate that memory replay based algorithm can be a very promising direction for large scale CL that should not be ignored.

We note that in Table~\ref{tab:taskonomy_1} that expansion based method Side-Tuning achieves zero forgetting and competitive performance drop. However, it requires a growing neural architecture which results in a large final model with more expensive inference cost. Its compute overhead will further increase when seeing larger numbers of tasks. After each task, Side-Tuning needs to add an additional side network which is also found expensive in the training storage cost. That prevents this method being applied to complex tasks that requires models with large capacity.

We also observe a degraded performance of vanilla experience replay with a small memory size, \textit{i.e.,} $m=64$ is worse than $m=256$. Although not surprising, the degraded performance inspired our study on the feature space which leads to the proposed improvement approach in the next section.

\footnotetext{This is the estimated training data size excluding the current task which needs access by multi-task learning.}
\footnotetext{EWC needs access to all previous tasks' encoder weights with the diagonal of fisher information.}

\vspace{-2mm}
\section{Compressed Activation Replay}
\vspace{-2mm}
Vanilla experience replay stores only input-output pairs and uses them to construct the replay loss. However, we suspect that, for large neural networks, intermediate features (activations) may undergo drifts when we train the model sequentially on different tasks. If that is the case, the input-output pairs may not be sufficient to mitigate this drift in the intermediate layers, leading to catastrophic forgetting. To better understand this phenomenon, we plot the t-SNE  \citep{tsne} visualization of the feature space over the course of vanilla ER in Figure~\ref{fig:tsne_ER}(a). We observe that indeed as new tasks are being learnt, feature representations of the older tasks start drifting. To circumvent this issue, we propose using feature matching as an additional regularization term.

%Since models in experience replay are regularized just using the task loss of older tasks, the regularization effect is perhaps insufficient to prevent the feature drift. 

%\subsection{Feature Space Visualization}


\input{figures/tsne}

% \subsection{Feature matching regularization}
Let $(\bx_r^j, \by_r^j)$ be a sample from task $j$, and let $\rvf_r^j = g(\bx_r^j)$ be the encoder representation (\textit{i.e.,} activation) of this sample at the end of the training of task $j$. The neural net prediction of this sample is thus $p^j(\bx_r^j) = h^j(\rvf_r^j)$. The basic idea of feature matching regularization is that, when we train a subsequent task, say task $i$, the encoder representation of the replay example $\bx_r^j$, \textit{i.e.,} $g(\bx_r^j)$ should stay close to $\rvf_r^j$. To achieve this, we add an additional regularization term $\ell_{fm}(g(\bx_r^j), \rvf_r^j)$ when training the subsequent tasks, where $\ell_{fm}$ is a loss function that measures the difference between $g(\bx_r^j)$ and $\rvf_r^j$. In the following, for most experiments we use a simple MSE loss, \textit{i.e.,} $\ell_{fm} (\rva, \rvb) \equiv \|\rva - \rvb\|_2^2$. In our ablation study in Section~\ref{sec:ablation}, we compare different choices of $\ell_{fm}$.


% Now, we write the second-order Taylor series expansion of the sample loss with respect to the encoder representation $\be = g(\bx)$.
% \begin{align}
%     \ell(h^i(\be), \by) - \ell(h^i(\be_0), \by) \approx (\be - \be_0)^\top \nabla_{\be} \ell(h^i(\be), \by) + \frac{1}{2} (\be - \be_0)^\top \bH (\be - \be_0),\label{eq:taylor}
% \end{align}
% where, $\bH$ is the Hessian of the loss.
% The above equation specifies the loss difference obtained due to the feature-space drift. The goal of continual learning is to minimize the quantity in Equation \ref{eq:taylor} for all examples. Directly computing this quantity may be computationally expensive. More generally, we can write the loss difference as a parametric function
% \begin{align*}
%     \ell(h^i(\be), \by) - \ell(h^i(\be_0), \by) =  (\be - \be_0)^\top A (\be - \be_0) + (\be - \be_0)^\top b.
% \end{align*}
% For different choices of $A$ and $b$, we obtain different regularizers. Specifically, if $A=I$ and $b=\mathbf{0}$, we obtain $\| \be - \be_0 \|^2_2$ which minimizes the Euclidean distance between the representations. We shall use this MSE regularizer in the rest of the paper. An ablation on using difference choices of feature matching losses are provided in Section [].

The activation tensors of intermediate layers in neural networks are usually of high dimensions, and storing them in the replay buffer can be expensive in memory cost. Since we also want to avoid too much overhead to the memory and compute cost, we empirically study a variant of feature matching regularization by compressing the activation into small-length vectors and only regularize the models in regards to such compressed vector representations. Formally, we use a compression function $c$ to map the high dimensional feature $\rvf_r^j$ to a low dimensional vector $c(\rvf_r^j)$, and then apply the feature matching loss $\ell_{fm}$. In this case, the feature matching loss for task $j$ can be written as
\begin{align}
    \cL^{j}_{fm} = \EE_{(\bx_{r}^{j}, \by_{r}^{j}, \rvf_{r}^{j}) \in \cM}~~ \ell_{fm}(c(g(\bx_{r}^j)), c(\rvf_{r}^j)),
\end{align}
and then the objective for training a subsequent task $i$ can then be written as 
\begin{align}
    \min_{g, h^i}~~ \cL^{i}_{task} + \frac{1}{i-1} \sum_{j=1}^{i-1} \left[ \lambda\cL^{j}_{replay} + \lambda_{fm} \cL^{j}_{fm} \right],
\end{align}
where $\lambda_{fm}$ is another coefficient balancing the feature matching loss and other terms in the loss function.
We name this approach Compressed Activation Replay (CAR). As presented in Figure~\ref{fig:tsne_ER}(b), by using CAR, the drift in the encoder representations is significantly reduced.
As for the compression function, a simple way to compress is to perform average pooling along axes (spatial and/or channel) of the tensors. Interestingly, we found this simple compression performs well in our experiments. In our ablation studies in Section~\ref{sec:ablation}, we compare different compression techniques.

% \subsection{Objective: } To perform feature matching, we need to store the feature representations $\be_0$ in addition to the input-output pairs. After training task $i$, for samples $(\bx_{r}^{i}, \by_{r}^{i})$ in the buffer $\cM$, we compute the feature representations $\be_{r}^i = g(\bx_{r}^{i})$ and store the resulting tuple $(\bx_{r}^i, \by_{r}^i, \be_{r}^i)$ in the replay buffer. The feature matching regularizer used while training task $i$ can then be written as
% \begin{align*}
%     \cL^{j}_{fm} = \EE_{(\bx_{r}^{j}, \by_{r}^{j}, \be_{r}^{j}) \in \cM}~~ \ell_{fm}(e(\bx_{r}^j), \be_{r}^j).
% \end{align*}
% Here, $\ell_{fm}(\cdot)$ is any feature matching loss function. The objective for training task $i$ can then be written as 
% \begin{align*}
%     \min_{g, h^i}~~ \cL^{i}_{task} + \frac{1}{i-1} \sum_{j=1}^{i-1} \left[ \lambda\cL^{j}_{replay} + \lambda_{fm} \cL^{j}_{fm} \right].
% \end{align*}
% which will be minimized as before.



\vspace{-2mm}
\section{Empirical studies}
% \vspace{-2mm}
\input{figures/prediction_vis}
% \vspace{-2mm}
\subsection{Taskonomy}
\vspace{-2mm}
We compare the proposed CAR approach with multiple baseline methods in the Taskonomy dataset mentioned in Section~\ref{sec:vanilla_er}: vanilla SGD, A-GEM, and vanilla experience replay (ER).
    % \item EWC: The elastic weight consolidation method which does not utilize a replay memory. The idea is to regularize the model weights with coefficients decided by the diagonal of the Fisher information matrix.
    % \item SideTuning \citep{sidetuning2020}: This method does not utilize a replay memory as well. For each new task, all the parameters trained from past tasks are frozen. A new side network is initialized and trained on the new task. The output of the new side network and the output of the past networks are concatenated to produce the final outputs of the model.
    % \item AGEM: This is an efficient variant of the Gradient Episodic Memory called Averaged Gradient Episodic Memory. During the training of each task, a batch of data is sampled from the episodic memory and the gradient w.r.t. these samples is computed using the current model. The gradient of the current task is projected into the orthogonal direction w.r.t. the gradient of the memory examples whenever they point towards the opposite directions.
    % \item ER: The vanilla experience replay method which uniformly samples data into a replay buffer and regularizes the output using the loss on these examples while training on the new tasks.

\input{tables/taskonomy.tex}

Two diferent task sequences are used in the evaluation. Results are shown in Table \ref{tab:taskonomy}. The trend in both task sequences are consistent where CAR significantly outperforms the other methods on the forgetting measure, \textit{e.g.}, it reduces forgetting rate of vanilla ER by $28\%$ when $m=64$. The performance drop of CAR is slightly higher but still comparable with ER. This can be explained by the stability-plasticity dilemma in continual learning~\citep{mermillod2013stability,mirzadeh2020understanding}, where, stability against forgetting is achieved at the slight cost in the plasticity of the model, \textit{i.e.}, the ability of  quickly acquiring new knowledge. The proposed feature matching loss acts as a regularizer and stabilizes the model resulting in a significant decrease in forgetting traded by a relatively smaller drop in learning new tasks. Nevertheless, the parameter $\lambda_{fm}$ is designed to control this trade-off and tune it according to the application. According to the tables, bigger memory size also improves the performance for the proposed CAR method. We visualize the model predictions  in Figure~\ref{fig:prediction_vis}, which show that the images predicted by CAR have higher quality than vanilla SGD and ER.

\vspace{-2mm}
\subsection{Split-CIFAR and Split-miniImageNet}
\vspace{-2mm}
In addition to the large-scale Taskonomy dataset, we perform experiments on two continual learning datasets - Split-CIFAR and Split-miniImageNet. We follow the protocol in \cite{chaudhry2020hindsightreplay, chaudhry2018efficient} for all the experiments -- Of the $20$ tasks in the task sequence, $3$ tasks are used for validation, while the other $17$ tasks are used to report the final performance. Each task is trained for a single epoch with a batch size of $10$.
Since each task is a $5$-way classification problem, we train models using cross-entropy loss. We use the reduced Resnet-18 model as the encoder following \cite{chaudhry2020hindsightreplay, chaudhry2018efficient}. Task heads are one-layer linear networks mapping the encoder layer to the logits.

In addition to the baselines listed previously, we also compare with the three additional replay based methods whose performance on Split-CIFAR and Split-miniImageNet were reported in the literature, i.e., iCaRL~\citep{Rebuffi_2017}, MER~\citep{riemer2018learning}, HAL~\citep{chaudhry2020hindsightreplay}.
\iffalse
\begin{enumerate}
\setlength\itemsep{0em}
    \item iCaRL~\citep{Rebuffi_2017} uses a nearest neighbor classifier based on the mean-of-exemplars. The catastrophic forgetting is reduced by means of knowledge distillation.
    \item MER~\citep{riemer2018learning}, called Meta Experience Replay, incorporates meta-learning objectives into an experience replay framework.
    \item HAL~\citep{chaudhry2020hindsightreplay} improves experience replay by learning an anchor representation for each task that maximizes its chance of forgetting. The anchor points are also stored in the replay memory and used to regularize the models in future training. 
\end{enumerate}
\fi

%\input{tables/split_cifar.tex}
%\input{tables/split_imagenet.tex}
\input{tables/std_benchmark}

The results on Split-CIFAR and Split-miniImageNet are shown in Table \ref{tab:split_cifar}. We found Compressed Activation Replay achieves significant improvement in CIFAR in terms of both final accuracy and forgetting rate. For Split-miniImageNet, our method outperforms all the methods significantly in the small memory case, and performs comparably to HAL in large memory case.

\subsection{Discussion}\label{sec:ablation}

\textbf{Compression techniques.} First, we compare the performance of different compression techniques used in CAR framework. Let the dimension of feature tensor be $(n_{f} \times w \times h)$. We employ the following simple compression schemes: (a) \textit{Spatial}: average pooling along the spatial dimension (dimension $n_{f}$); (b) \textit{Channel}: average pooling along the channel dimension (dimension $wh$); (c) \textit{Spatial + Channel}: a concatenation of spatial and channel pooling (dimension $n_f+wh$).

\input{tables/taskonomy_compression.tex}
\iffalse
\begin{enumerate}
\setlength\itemsep{0em}
\item Spatial: average pooling along the spatial dimension (feature dimension $n_{f}$).

\item Channel: average pooling along the channel dimension (feature dimension $wh$).

\item Spatial + Channel: a concatenation of spatial and channel pooling (dimension $n_f+wh$).

\end{enumerate}
\fi

In addition to performance, we report in Table.~\ref{tab:taskonomy_compression} the memory overhead needed for storing the samples in the replay buffer. With significantly lower memory overhead, compression techniques perform comparably to those without compression. Among the compression methods, channel pooling performs poorly compared to spatial pooling. Spatial+Channel pooling achieves the best result. 



\textbf{Regularization functions.}
We compare different regularization functions $\ell_{fm}$ for feature matching. Natural choices are $\ell_2$ and $\ell_1$ distances. Besides that we also experiment with weighted version of $\ell_1$ and $\ell_2$ where the weights are computed by accumulating the gradients, since neurons with high magnitude of changes are often important to the corresponding tasks. In addition, we also tried the MMD loss~\citep{gretton2007kernel}, a popular distribution matching distance. Interestingly, none of them is significantly better than the rest. Detailed results can be found in Appendix.

\vspace{-2mm}
\section{Conclusion}
\vspace{-2mm}
We studied the large scale continual learning using memory replay based methods on a non-conventional diverse set of tasks.
We compared the performance of different  methods in both Taskonomy and medium-scale CIFAR/miniImageNet datasets and found that vanilla experience replay is a strong baseline algorithm despite its simplicity. However, feature drift is observed while training with a standard replay memory.
We further proposed the Compressed Activation Replay framework, which aims to reduce such drifting. Experimental results show that our approach achieves the state-of-the-art performance on both large scale Taskonomy benchmark and standard medium-size continual learning datasets.

==> compressed activation replay ICLR 2021/figures/prediction_vis.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/Prediction_vis.pdf}
\caption{\small Visualizations of predictions made on Taskonomy dataset. Compressed Activation Replay (CAR) drives the predictions to higher quality, compared with vanilla SGD and ER.}
\vspace{-4mm}
\label{fig:prediction_vis} 
\end{figure*}

==> compressed activation replay ICLR 2021/figures/title_fig.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figures/ICLR_CAR_title_fig_with_embeddings_v2.pdf}
\caption{\small\textbf{Compressed Activation Replay (CAR)}: During sequential training, compressed feature maps are stored in addition to the input-output pairs in the replay buffer. While training future tasks, models are optimized using (1) task loss, (2) replay task loss using samples from the replay buffer and (3) activation matching loss between the compressed activation maps of the current encoder model and the replay samples. Activation matching loss present distribution drift from happening in the feature space.}
\label{fig:title_fig} 
\end{figure*}

==> compressed activation replay ICLR 2021/figures/tsne.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figures/t-SNE_joint.pdf}
\vspace{-2mm}
\caption{\small\textbf{Visualizing t-SNE embeddings} of model trained using vanilla experience replay (a) and Compressed Activation Replay (b) on Split-CIFAR dataset. We compare the features of the encoder of the final model (\emph{shown in blue}) relative to the encoder representations obtained while training the respective tasks (\emph{shown in red}). We observe that older tasks encounter significant drift in the feature space when trained with experience replay. Using activation matching loss, our Compressed Activation Replay framework reduces the drift as the blue dots better cover the support of red dots, especially on Task 5 and 10. We note that for the very early task (Task 0), feature drift can still be observed even if we use CAR.
}
\vspace{-4mm}
\label{fig:tsne_ER} 
\end{figure*}

==> compressed activation replay ICLR 2021/figures/tsne_CAER.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/TSNE_plot_FM.png}
\caption{\textbf{Visualizing t-SNE embeddings} of model trained using Compressed Activation Replay on Split-CIFAR dataset. We compare the features of the encoder of the final model (\emph{shown in blue}) relative to the encoder representations obtained while training the respective tasks (\emph{shown in red}). Feature space drift on older tasks are significantly reduced compared to experience replay (Figure~\ref{fig:tsne_ER}). }
\label{fig:tsne_CAER} 
\end{figure*}

==> compressed activation replay ICLR 2021/intro.tex <==
\begin{abstract}
% We study the continual learning problem in a large scale setting where sequential tasks are not limited to classification and the output can be of high dimensions. Based on a study of various state-of-the-art methods, we found memory replay tends to be more effective, in terms of both performance and scalability. While most existing methods only replay the input-output pairs, the regularization effect may not be sufficient for complex deep models. Inspired by this intuition, we propose to also replay the activation of the intermediate layer of neural networks. Directly saving the activation can dramatically increase the memory and compute cost. Instead, we propose the Compressed Activation Replay framework, which uses a tiny compressed version of layer activation. We show that this approach can achieve superior regularization performance while adding up negligible memory cost in the replay buffer. We compare our approach with existing methods on standard datasets such as Split CIFAR and Split mini-Imagenet. Significantly improved continual learning capability is observed in the large scale Taskonomy benchmark.

We study continual learning in the large scale setting where tasks in the input sequence are not limited to classification, and the outputs can be of high dimension. Among multiple state-of-the-art methods, we found vanilla experience replay (ER) still very competitive in terms of both performance and scalability, despite its simplicity.
However, a degraded performance is observed for ER with small memory. A further visualization of the feature space reveals that the intermediate representation undergoes a distributional drift.
While existing methods usually replay only the input-output pairs, we hypothesize that their regularization effect is inadequate for complex deep models and diverse tasks with small replay buffer size. Following this observation, we propose to replay the activation of the intermediate layers in addition to the input-output pairs. Considering that saving raw activation maps can dramatically increase memory and compute cost, we propose the Compressed Activation Replay technique, where compressed representations of layer activation are saved to the replay buffer. We show that this approach can achieve superior regularization effect while adding negligible memory overhead to replay method. Experiments on both the large-scale Taskonomy benchmark with a diverse set of tasks and standard common datasets (Split-CIFAR and Split-miniImageNet) demonstrate the effectiveness of the proposed method.

\end{abstract}

\section{Introduction}
Humans naturally learn concepts and tasks in a sequential order without degrading performance on the previous ones. Can machines do the same?
This setting, known as \textit{continual learning}, poses serious challenges for the deep learning community.
Deep neural networks often fail to maintain the performance on the previous tasks if they cannot fully access their data, a phenomenon called \textit{catastrophic forgetting}. The underlying cause is the assumption that models learn from \emph{i.i.d.} (independent and identical distributed) data. This assumption is often untrue in the real world where data can come sequentially and their distributions can always be evolving.
The solution to this issue will be a key to a system that allows machines to learn continuously in the real world.

% This setting called \textit{Continual Learning} posses serious challenges for  deep learning among which the phenomena of \textit{Catastrophic Forgetting} is the most critical. It states that the models fail to maintain the previous performance if they cannot fully access old data.


As the machine learning models become deeper and wider while the size of the data gets bigger and the tasks become more diverse, the catastrophic forgetting issue becomes more significant and concerning. In recent years, much work has been proposed to address the forgetting problem. However, existing continual learning methods are usually developed and evaluated on relatively small datasets, often with classification tasks only. The scalability of these methods and their effectiveness in real scenarios with a diverse pool of tasks are still an open question and often being overlooked.



%A major factor that distinguishes all the continual learning methods is whether they save examples of the past tasks, \emph{a.k.a.} replay examples or not. 
The first question we want to study is: \textit{how different classes of methods work in large scale continual learning with a diverse set of tasks?} We conduct a systematic evaluation of various continual learning algorithms using a comprehensive multi-task benchmark based on the Taskonomy dataset~\citep{zamir2018taskonomy}. This dataset contains not only classification tasks but also regression with high dimensional outputs. Interestingly, we observe in this large scale setting that the vanilla memory replay method outperforms a variety of state-of-the-art approaches, based on a range of evaluation protocols using forgetting reduction, generalization, scalability and inference efficiency.

\input{figures/title_fig}

%Two factors are considered here: (1) the sampling strategy, and (2) the input-output pairs fore replay. We suspected that uniform sampling may not be the most effective sampling approach because the number of samples in a memory is small so it may be difficult to fully capture the past data distribution. Therefore, the second question we want to answer is: \textit{how important is the sampling strategy for the replay buffer?} Somewhat surprisingly, after investigating multiple sampling strategies (such as class-balancing methods), we found that uniform sampling performs generally the best on Taskonomy dataset. This shows that on large scale datasets with diverse set of tasks and high dimensional regression tasks, uniform sampling is already a competitive approach, and designing more sophisticated sampling approaches may only provide marginal, if any, gain on these datasets.

Though being competitive, we observe a degraded performance of vanilla experience replay with a small memory size. A t-SNE plot of the feature space, illustrated in Fig.~\ref{fig:title_fig} top middle, reveals that the intermediate representation still undergoes a distributional shift. We believe it is due to the fact that most replay methods store and regularize using only the input-output pairs from past tasks. Considering that modern neural networks are often wide and deep, we argue that replaying only the input-output pairs are not enough to constrain the feature space. A natural solution is to augment the replay memory with the activation of intermediate layers to regularize representation learning. 

%In order to further improve their performance, we study a second research question as \textit{Whether input-output pairs are sufficient for an effective replay of past experience?}
%We also considered the effectiveness of constructing the replay loss by posing the third research question: \textit{What are the effective input output pairs for the sake of replay?}.
%Our deriving motivation is the observation that the intermediate representations usually undergo drifts as we learn new tasks schematically shown in Fig.~\ref{fig:title_fig} top middle box.
%Due to the fact that modern neural networks are generally wide and deep, replaying only the input-output pairs may result in large variance, instability, and reduced effect in the intermediate layers. 
%A natural idea is to augment the replay memory with intermediate activation of the neural networks to regularize the representation learning. 

However, given the size of models used in large scale scenarios, these activation tensors can be very expensive in terms of both memory and computation cost. Therefore, we propose a \emph{Compressed Activation Replay (CAR)} framework which regularizes the model by matching the compressed versions of those activation tensors (Fig.~\ref{fig:title_fig}). The chosen compression function is based on average pooling along both spatial and channel dimensions, which results in negligible added compute cost compared to vanilla memory replay. Experimental results also suggest that the compressed replay approach produces equivalent performance compared to replaying the full activation tensors, and outperforms the baseline replay algorithm that only replays the raw input-output pairs.

We evaluate our approach on the large scale Taskonomy benchmark to demonstrate its scalability. New performance evaluation metrics are proposed to tailor the need of large scale setups with diverse tasks. In order to compare with other methods in literature, we also conduct experiments on two medium-sized popular datasets, \textit{i.e.}, Split-CIFAR and Split-miniImageNet. Empirical results suggest that our approach achieves the state of the art in all three benchmarks.

In summary, our contributions are as follows:
% \begin{enumerate}
% \setlength\itemsep{0em}
% %\setlength\itemindent{-2em}
%     \item We provide an empirical study that shows simply replay is still a strong baseline in large scale continual learning, even compared with the sophisticated state-of-the-art alternatives.
%     \item We provide a comparative study with various sampling strategies for filling the replay buffer, the result of which shows that uniform sampling is still a competitive strategy.
%     \item We propose a novel and effective replay approach which regularizes the model using a compressed representation of intermediate layer activation in neural networks.
% \end{enumerate}
\begin{enumerate}%[leftmargin=*]
\setlength\itemsep{0em}
    \item We provide a thorough evaluation of popular continual learning methods at a large scale with diverse tasks which is mostly missing in the published literature.
    \item We show the vanilla experience replay is the most effective approach in the large scale setting in the presence of task diversity.
    \item We observe that intermediate representations still undergo a drift in continual learning process reinforcing the catastrophic forgetting. 
    \item We propose Compressed Activation Replay (CAR) to improve the performance of experience replay, reaching state-of-the-art results among replay based methods.
\end{enumerate}

\section{Related work}\label{sec:related_work}
\textbf{Catastrophic forgetting.} Catastrophic forgetting is a major challenge in deep learning where the performance of past examples may drop significantly in a sequential training setting. Continual learning aims to address this problem. The approaches are often categorized into three major directions: replay, expansion and regularization based methods. Replay based methods require a memory module to memorize past or generative examples (see next paragraph for more discussion). Regularization methods are achieved by introducing regularization terms into the loss function which constraint the model weights~\citep{Kirkpatrick_2017,zenke2017continual,ritter2018online,farajtabar2019orthogonal,yin2020sola,Adel2020ContinualLW}. Expansion based methods
%such as Progressive Neural Network 
\citep{rusu2016progressive,li2017learning,yoon2018lifelong,li2019learn,mirzadeh2020dropout} tackle the problem by expanding the neural architecture along the training. Specifically, the predictive capability on the past examples is retained by freezing the architecture related to past tasks while the new examples are further trained with an extended set of network parameters. These approaches need to expand the neural network, leading to large models in the end. Lacking a proper way for parameter sharing, most of the expansion based methods are found hard to be applied to large scale tasks. 

%Elastic weight consolidation (EWC) \citep{Kirkpatrick_2017} adds a quadratic penalty of the weights w.r.t. the final weights from the previous task. The diagonal of the Fisher information matrix is incorporated in this penalty. Recent work by \cite{yin2020sola} derives the regularization by approximating the loss from the previous task. Taylor expansion of the loss implies that Hessian approximation is the key to a proper loss reconstruction. The paper also suggests that EWC is a special case since the Fisher information matrix is equivalent to the Hessian of the log-likelihood loss.

\textbf{Memory replay methods.}
Mitigating catastrophic forgetting via memory replay is a classic idea that dates back to the 90s~\citep{robins1995catastrophic}. These methods typically save a sampled set of input-output pairs into a memory module and mix these samples with new samples in the current task for training the models.
It has been observed that replay based algorithms usually outperform regularization based methods~\citep{nguyen2017variational,van2019three}, and some explanation have been made by~\cite{knoblauch2020optimal}. Among replay based methods, some try to design new update rules using replay samples~\citep{lopez2017gradient,chaudhry2018efficient}, while others focus on new sampling strategies to fill the replay buffer~\citep{Rebuffi_2017,chaudhry2020hindsightreplay,aljundi2019gradient,Hayes_2019,chrysakis2020online,borsos2020coresets}. Another line of research uses generative models to construct replay examples~\citep{shin2017continual,van2020brain}. Replaying the experience is also popular in reinforcement learning problems \citep{mnih2013playing,schaul2015prioritized,isele2018selective,rolnick2019experience}.

One recent work that is particularly related to our proposed approach is the embedding regularization algorithm~\citep{pomponi2020efficient}. In this algorithm, the network embedding of replay examples are stored in memory and a regularization loss is constructed using the embedding such that the feature extraction layers remain stable. While the basic idea of this work is similar to our proposed method, we differentiate in two ways: 1) in our proposed Compressed Activation Replay method, only a compressed version of the network embedding is stored in the replay buffer, which significantly reduces the memory cost without sacrificing the regularization effect, and 2) we benchmark the performance of the approach on large scale non-classification tasks such as Taskonomy, whereas~\cite{pomponi2020efficient} only provides results based on MNIST and CIFAR.

% \dong{Once we finalize the algorithm, we need to check back this paragraph and see if the comparison with embedding regularization is still accurate.}


\textbf{Large scale continual learning.} Most existing continual learning literature still focuses on evaluations on small-scale dataset such as MNIST and CIFAR. The Taskonomy dataset~\citep{zamir2018taskonomy} has been used recently for continual learning study in \citep{sidetuning2020}, where they propose the Side-Tuning algorithm to mitigate catastrophic forgetting. Side-Tuning is an expansion based method, which trains a separate side network for every new tasks and blend the output of the side network with that of the previous frozen networks. The method is able to achieve zero forgetting since all previous tasks' models are frozen. A potential concern for this method is that the inference time of later tasks is significantly higher than that of earlier tasks. Our proposed approach differs from Side-Tuning in that we allow the representation network to be shared and evolved over tasks with stable model capacity and inference time.
Another large scale dataset that is often used in continual learning research is the CORe50 dataset~\citep{lomonaco2017core50}, which mainly focuses on object detection. In this work, we choose Taskonomy since it contains more diverse tasks.

==> compressed activation replay ICLR 2021/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\dong}[1]{{\color{brown} dong: #1}}
\newcommand{\ang}[1]{{\color{blue} ang: #1}}
\newcommand{\mehrdad}[1]{{\color{magenta} Mehrdad: #1}}

==> compressed activation replay ICLR 2021/tables/cifar_255_results.tex <==
\begin{table*}[ht]
\caption{\small\textbf{Split-CIFAR and Split-miniImageNet Results:}  Average accuracy (acc$\pm$std \%) and forgetting ($\pm$std) values are reported. Results are averaged over $5$ random seeds. The best result is highlighted in bold.}
\label{tab:split_cifar_255}
\begin{center}
%\resizebox{\textwidth}{!}{
\begin{tabular}{r|cc|cc}
\toprule
& \multicolumn{2}{|c||}{\sc Split-CIFAR} & \multicolumn{2}{c}{\sc Split-miniImageNet}\\
Method & \multicolumn{2}{c}{$m=255$} & \multicolumn{2}{c}{$m=255$} \\  
 & \it {acc}($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$)  & \it fgt($\downarrow$)  \\
 \midrule \midrule 
 iCaRL  &  51.7\std{1.4} & 0.13\std{0.02} &  - &  - \\
 A-GEM   &  56.9\std{3.4} & 0.13\std{0.03} & 51.6\std{2.6} & 0.10\std{0.02} \\
 MER    &  57.7\std{2.6} & 0.11\std{0.01} &  49.4\std{3.4} & 0.12\std{0.02} \\
 ER     &  60.9\std{1.4} & 0.09\std{0.01} &  53.5\std{1.4} & 0.07\std{0.02}  \\
 HAL    &  62.9\std{1.5} & 0.08\std{0.01} & \bf 56.5\std{0.8} & \bf 0.06\std{0.01} \\
 \midrule
 CAR (ours)  & \bf 65.2\std{2.1} &  \bf 0.05\std{0.01} & 55.1\std{2.1} & \bf 0.06\std{0.01}  \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> compressed activation replay ICLR 2021/tables/sensitivity_analysis.tex <==
\begin{table*}[ht]
\caption{\textbf{Sensitivity of $\lambda_{fm}$:} Forgetting (\textit{fgt}) and performance drop ($\Delta$\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
\label{tab:taskonomy_sensitivity_analysis}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l |cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
 & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & $\Delta$\textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) \\
 \midrule 
 \midrule
 $\lambda_{fm} = 0.25$ & 32.57 & 25.36 & 24.09 & 19.06 & 15.79 & 11.49 & 9.06 & 13.84\\
 $\lambda_{fm} = 1.0$  & 28.49 & 25.33 & 20.45 & 20.91 & 11.24 & 17.83 & 7.09 & 12.89 \\
 $\lambda_{fm} = 5.0$  & 25.19 & 29.06 & 12.01 & 18.46 & 8.26 & 17.03 &  2.18 & 10.44 \\
 $\lambda_{fm} = 20.0$ & 18.21 & 24.72 & 10.09 & 18.86 & 4.29 & 12.43 &  -0.29 & 14.94 \\
 $\lambda_{fm} = 50.0$ & 13.37 & 23.25 & 6.25 & 19.32  & 2.13 & 20.17 &  -1.65 & 17.29\\
 
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


%% Sensitivity of Split-CIFAR

\begin{table*}[ht]
\caption{\textbf{Sensitivity of $\lambda_{fm}$:} Average accuracy (in \%) and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cifar_sensitivity}
\begin{center}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
 & \multicolumn{4}{|c|}{Split-CIFAR} & \multicolumn{4}{|c}{Split-miniImagenet} \\  
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=425$} & \multicolumn{2}{|c}{$m=85$} & \multicolumn{2}{|c}{$m=425$} \\  
 & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} \\
\midrule
 $\lambda_{fm}=0.25$  & 59.0 & 0.09 & 64.4 & 0.06 & 50.9 & 0.08 & 53.6 & 0.08 \\
 $\lambda_{fm}=1.0$   & 61.4 & 0.07 & 65.3 & 0.05 & 53.3 & 0.07 & 54.2 & 0.07 \\
 $\lambda_{fm}=5.0$   & 62.4 & 0.06 & 66.5 & 0.04 & 54.2 & 0.06 & 56.2 & 0.06 \\
 $\lambda_{fm}=10.0$  & 62.0 & 0.06 & 66.0 & 0.03 & 53.3 & 0.06 & 53.4 &  0.07 \\
 $\lambda_{fm}=25.0$  & 62.2 & 0.06 & 63.3 & 0.03 & 52.2 & 0.07 & 51.5 &  0.05 \\
 $\lambda_{fm}=100.0$ & 58.6 & 0.04 & 55.8 & 0.02 & 46.1 & 0.04 & 42.3 &  0.03 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/split_cifar.tex <==
\begin{table*}
\caption{\textbf{Split-CIFAR Results:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cifar}
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=255$} & \multicolumn{2}{|c}{$m=425$} \\  
 & Accuracy & Forgetting & Accuracy  & Forgetting & Accuracy & Forgetting \\
 \midrule \midrule 
 EWC    & 42.4 & 0.25 & - & - & - & - \\


 ICARL  & 46.4 & 0.16 & 51.7 & 0.13 & 51.2 & 0.13 \\
 AGEM   & 54.9 & 0.14 & 56.9 & 0.13 & 59.9 & 0.10 \\
 MER    & 49.7 & 0.19 & 57.7 & 0.11 & 60.6 & 0.09 \\
 ER     & 56.2 & 0.13 & 60.9 & 0.09 & 62.6 & 0.06 \\
 HAL    & 60.4 & 0.10 & 62.9 & 0.08 & 64.4 & 0.06 \\
 \midrule
 CAR (ours)  & 62.4 &  0.06 & 65.2 &  0.05 & 66.5 &  0.04 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/split_cifar_experiment_details.tex <==
\begin{table*}
\caption{\textbf{Experiment details on Split-CIFAR / Split-miniImageNet dataset}}
\label{tab:exp_details_split_cifar}
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l}
\toprule
    Encoder Architecture    & Resnet-18 used in \cite{chaudhry2018efficient} \\
    Task head               & FC layer \\
    Encoder Learning rate   & 0.03    \\
    Task head rate          & 0.03    \\
    Optimizer               & SGD      \\
    LR Decay                & None      \\
    Batch Size              & 10        \\
    Number of training iterations    & Single epoch training    \\
    
    \midrule
    \multicolumn{2}{c}{Experience Replay} \\
    \midrule
    Buffer filling strategy & Uniform Sampling \\
    Replay batch size       & 5 \\
    
    \midrule
    \multicolumn{2}{c}{CAR} \\
    \midrule
    Regularization function $\ell_{fm}$ & MSE loss \\
    Compression scheme      & No compression used \\
    $\lambda_{fm}$          & 5.0 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/split_cls_buffer_filling.tex <==
\begin{table*}
\caption{\textbf{Buffer filling techniques:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cls_buffer_filling}
\begin{center}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|cc|cc  ||  cc|cc}
\toprule
 & \multicolumn{4}{|c||}{Split-CIFAR} & \multicolumn{4}{|c}{Split-miniImagenet} \\  
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c||}{$m=425$} & \multicolumn{2}{|c}{$m=85$} & \multicolumn{2}{|c}{$m=425$} \\  
 & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} \\
\midrule
 Reservoir Sampling & 56.1 & 0.12 & 63.4 & 0.07 & 50.0 & 0.09 & 53.2 & 0.08 \\
 Hard Example Mining & 45.1 & 0.22 & 55.0 & 0.14 & 39.4 & 0.18 & 45.4 & 0.14 \\
 Easy Example Mining & 56.6 & 0.09 & 64.1 & 0.06 & 50.0 & 0.08 & 55.4 & 0.06 \\
 High Variance Filling & 56.4 & 0.12 & 63.7 & 0.07 & 50.6 & 0.08 & 52.6 & 0.09 \\
 Loss Equilization & 49.6 & 0.19 & 61.4 & 0.09 & 45.6 & 0.13 & 53.0 & 0.08 \\
 Loss Equilization (importance) & 52.1 & 0.16 & 61.6 & 0.08 & 45.4 & 0.13 & 52.2 & 0.09 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/split_cls_distribution_matching.tex <==
\begin{table*}[ht]
\caption{\textbf{Distribution Matching Techniques}  Average accuracy (in \%) and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cls_distribution_matching}
\begin{center}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
 & \multicolumn{4}{|c|}{Split-CIFAR} & \multicolumn{4}{|c}{Split-miniImageNet} \\  
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=425$} & \multicolumn{2}{|c}{$m=85$} & \multicolumn{2}{|c}{$m=425$} \\  
 & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} \\
\midrule
 $\ell_{1}$ & 62.4 & 0.07 & 66.1 & 0.04 & 54.1 & 0.07 & 55.4 & 0.07   \\
 $\ell_{2}$ & 62.4 & 0.07 & 66.4 & 0.04 & 53.8 & 0.06 & 56.3 & 0.06 \\
 $\ell_{1} + \ell_{2}$ & 62.0 & 0.07 & 66.1 & 0.04 & 53.5 & 0.07 & 56.4 & 0.06  \\
 Weighted $\ell_{1}$ &  63.2 & 0.06 & 67.1 &  0.04 & 54.6 & 0.06 & 55.8 & 0.07   \\
 Weighted $\ell_{2}$ & 61.5 & 0.07 & 67.0 & 0.04 & 53.8 & 0.06 & 56.3 & 0.07   \\
 MMD & 56.4 & 0.11 & 63.2 & 0.06 & 51.2 & 0.08 & 55.0 & 0.08 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/split_imagenet.tex <==
\begin{table*}
\caption{\textbf{Split-miniImagenet Results:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_miniimagenet}
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=255$} & \multicolumn{2}{|c}{$m=425$} \\  
 & Accuracy & Forgetting & Accuracy  & Forgetting & Accuracy & Forgetting \\
 \midrule \midrule 
 EWC    & 37.7 & 0.21 & - & - & - & - \\


 AGEM   & 48.2 & 0.13 & 51.6 & 0.10 & 54.3 & 0.08 \\
 MER    & 45.5 & 0.15 & 49.4 & 0.12 & 54.8 & 0.07 \\
 ER     & 49.0 & 0.12 & 53.5 & 0.07 & 54.2 & 0.08 \\
 HAL    & 51.6 & 0.10 &  56.5 &  0.06 &  57.2 &  0.06 \\
 \midrule
 CAR (ours)  &  54.2 &  0.06 & 55.1 &  0.06 & 56.2 &  0.06 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/std_benchmark.tex <==
% \begin{table*}
% \caption{\small\textbf{Split-CIFAR and Split-miniImageNet Results:}  Average accuracy (acc$\pm$std \%) and forgetting ($\pm$std) values are reported. Results are averaged over $5$ random seeds. The best result is highlighted in bold.}\vskip -1em
% \label{tab:split_cifar}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|cc|cc|cc||cc|cc|cc}
% \toprule
% & \multicolumn{6}{|c||}{\sc Split-CIFAR} & \multicolumn{6}{c}{\sc Split-miniImageNet}\\
% Method & \multicolumn{2}{c}{$m=85$}  & \multicolumn{2}{c}{$m=255$} & \multicolumn{2}{c||}{$m=425$} &\multicolumn{2}{c}{$m=85$}  & \multicolumn{2}{c}{$m=255$} & \multicolumn{2}{c}{$m=425$} \\  
%  & \it {acc}($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$)  & \it fgt($\downarrow$) & \it acc($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$)  & \it fgt($\downarrow
%  $) & \it acc($\uparrow$) & \it fgt($\downarrow$) \\
%  \midrule \midrule 
%  EWC    & 42.4\std{3.0} & 0.25\std{0.02} & - & - & - & -  & 37.7 & 0.21 & - & - & - & -\\


%  iCaRL  & 46.4\std{1.2} & 0.16\std{0.01} & 51.7\std{1.4} & 0.13\std{0.02} & 51.2\std{1.3} & 0.13\std{0.02} & - & - & - & - & - & - \\
%  A-GEM   & 54.9\std{2.9} & 0.14\std{0.03} & 56.9\std{3.4} & 0.13\std{0.03} & 59.9\std{2.6} & 0.10\std{0.02} & 48.2\std{2.4} & 0.13\std{0.02} & 51.6\std{2.6} & 0.10\std{0.02} & 54.3\std{1.6} & 0.08\std{0.01}\\
%  MER    & 49.7\std{2.9} & 0.19\std{0.03} & 57.7\std{2.6} & 0.11\std{0.01} & 60.6\std{2.1} & 0.09\std{0.02} & 45.4\std{1.4} & 0.15\std{0.01} & 49.4\std{3.4} & 0.12\std{0.02} & 54.8\std{1.7} & 0.07\std{0.01} \\
%  ER     & 56.2\std{1.9} & 0.13\std{0.01} & 60.9\std{1.4} & 0.09\std{0.01} & 62.6\std{1.8} & 0.06\std{0.01} & 49.0\std{2.6} & 0.12\std{0.02} & 53.5\std{1.4} & 0.07\std{0.02} & 54.2\std{3.2} & 0.08\std{0.02} \\
%  HAL    & 60.4\std{0.5} & 0.10\std{0.01} & 62.9\std{1.5} & 0.08\std{0.01} & 64.4\std{2.1} & 0.06\std{0.01} & 51.6\std{2.0} & 0.10\std{0.01} & \bf 56.5\std{0.8} & \bf 0.06\std{0.01} & \bf 57.2\std{1.5} & \bf 0.06\std{0.01}\\
%  \midrule
%  CAR (ours)  & \bf 62.4\std{1.5} & \bf 0.06\std{0.01} &\bf 65.2\std{2.1} &  \bf 0.05\std{0.01} & \bf 66.5\std{1.8} &  \bf 0.04\std{0.01} & \bf 54.2\std{2.9} & \bf 0.06\std{0.01} & 55.1\std{2.1} & \bf 0.06\std{0.01} & 56.2\std{1.8} & \bf 0.06\std{0.01} \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-4mm}
% \end{center}
% \end{table*}


\begin{table*}
\caption{\small\textbf{Split-CIFAR and Split-miniImageNet results:}  Average accuracy (acc$\pm$std \%) and forgetting ($\pm$std) values are reported. Results are averaged over $5$ random seeds. The best result is highlighted in bold.}\vskip -1em
\label{tab:split_cifar}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|cc|cc|cc|cc}
\toprule
& \multicolumn{4}{|c|}{\sc Split-CIFAR} & \multicolumn{4}{c}{\sc Split-miniImageNet}\\
Method & \multicolumn{2}{c}{$m=85$}  & \multicolumn{2}{c|}{$m=425$} &\multicolumn{2}{c}{$m=85$}  &  \multicolumn{2}{c}{$m=425$} \\  
 & \it {acc}($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$) & \it fgt($\downarrow$) & \it acc($\uparrow$)  & \it fgt($\downarrow
 $) \\
 \midrule \midrule 
 EWC    & 42.4\std{3.0} & 0.25\std{0.02} & - & -  & 37.7\std{3.3} & 0.21\std{0.03} & - & -\\


 iCaRL  & 46.4\std{1.2} & 0.16\std{0.01} & 51.2\std{1.3} & 0.13\std{0.02} & - & - & - & - \\
 A-GEM   & 54.9\std{2.9} & 0.14\std{0.03} & 59.9\std{2.6} & 0.10\std{0.02} & 48.2\std{2.4} & 0.13\std{0.02}  & 54.3\std{1.6} & 0.08\std{0.01}\\
 MER    & 49.7\std{2.9} & 0.19\std{0.03} & 60.6\std{2.1} & 0.09\std{0.02} & 45.4\std{1.4} & 0.15\std{0.01}  & 54.8\std{1.7} & 0.07\std{0.01} \\
 ER     & 56.2\std{1.9} & 0.13\std{0.01} & 62.6\std{1.8} & 0.06\std{0.01} & 49.0\std{2.6} & 0.12\std{0.02}  & 54.2\std{3.2} & 0.08\std{0.02} \\
 HAL    & 60.4\std{0.5} & 0.10\std{0.01} & 64.4\std{2.1} & 0.06\std{0.01} & 51.6\std{2.0} & 0.10\std{0.01} & \bf 57.2\std{1.5} & \bf 0.06\std{0.01}\\
 \midrule
 CAR (ours)  & \bf 62.4\std{1.5} & \bf 0.06\std{0.01} & \bf 66.5\std{1.8} &  \bf 0.04\std{0.01} & \bf 54.2\std{2.9} & \bf 0.06\std{0.01} & 56.2\std{1.8} & \bf 0.06\std{0.01} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/taskmonomy_intermediate.tex <==
\begin{table*}[ht]
\caption{\textbf{Effect of using intermediate representations:} Forgetting (\textit{fgt}) and performance drop ($\Delta$\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
\label{tab:taskonomy_intermediate}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l |cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
 & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) \\
 \midrule 
 \midrule
 CAR  & 13.37 & 23.25 & 4.80 & 17.32 & 2.98 & 12.43 & 1.91 & 11.51 \\
 CAR (\textit{intermediate}) & 15.44 & 22.17 & 8.75 & 19.01 & 3.53 & 14.84 & 0.58 & 13.59 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> compressed activation replay ICLR 2021/tables/taskonomy.tex <==

\begin{table*}
\caption{\small\textbf{Taskonomy results} using various replay methods. Forgetting (\textit{fgt}$\pm$std) and performance drop ($\Delta$\textit{perf}$\pm$std) values are reported (smaller values are better). All results are averaged over $3$ random seeds.}
\vskip -1em
\label{tab:taskonomy}
\setlength\tabcolsep{3pt}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{c|}{$m=64$}  & \multicolumn{2}{c|}{$m=128$} & \multicolumn{2}{c|}{$m=256$} & \multicolumn{2}{c}{$m=512$} \\  
 & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) \\
 \midrule 
 \multicolumn{9}{l}{\it {Sequence}: \small \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
\midrule
 SGD  & 191.6\std{13.8} & 101.6\std{9.2} & 191.6\std{13.8} & 101.6\std{9.2} & 191.6\std{13.8} & 101.6\std{9.2} & 191.6\std{13.8} & 101.6\std{9.2} \\
 A-GEM   &  43.6\std{0.7} & 48.0\std{0.9} & 44.1\std{2.3} & 50.2\std{2.8} & 38.9\std{1.9} & 49.0\std{2.9} & 24.9\std{3.1} & 50.9\std{4.7} \\
 ER     &  40.2\std{1.9} & 20.7\std{0.5} & 24.7\std{1.4} & 13.8\std{0.7} & 14.7\std{3.1} & 8.5\std{0.5} & 8.3\std{0.8} &  5.4\std{2.4} \\
CAR (ours) &   13.4\std{3.6} & 23.3\std{2.8} & 6.3\std{0.7} & 19.3\std{3.1} & 4.3\std{0.2} & 12.4\std{3.8} &  2.2\std{0.8} & 10.8\std{2.2} \\
 \midrule
 \multicolumn{9}{l}{\it {Sequence}: \small\textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
\midrule
 SGD  & 110.5\std{16.3} & 79.5\std{14.3} & 110.5\std{16.3} & 79.5\std{14.3} & 110.5\std{16.3} & 79.5\std{14.3} & 110.5\std{16.3} & 79.5\std{14.3} \\
 A-GEM   &  46.5\std{4.3} & 64.0\std{4.9} & 48.9\std{3.0} & 62.3\std{4.0} & 46.7\std{4.8} & 71.7\std{4.9} & 32.6\std{5.1} & 60.1\std{5.7} \\
 ER  &  43.8\std{2.7} & 33.4\std{3.2} & 24.0\std{4.5} & 24.3\std{3.2} & 19.9\std{6.4} & 12.7\std{4.5} & 9.1\std{3.9} &  5.3\std{2.9} \\
CAR (ours) & 15.9\std{4.6} & 35.6\std{3.1} & 7.9\std{2.6} & 26.8\std{4.5} & 6.7\std{1.2} & 14.3\std{0.7} & 5.7\std{3.1} & 10.8\std{1.1} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{center}
\end{table*}


% below is the original table with double digit.
\iffalse
\begin{table*}
\caption{\small\textbf{Taskonomy results} using various replay methods. Forgetting (\textit{fgt}$\pm$std) and performance drop ($\Delta$\textit{perf}$\pm$std) values are reported (smaller values are better). All results are averaged over $3$ random seeds.}

\label{tab:taskonomy_double_digit}
\setlength\tabcolsep{5pt}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{c|}{$m=64$}  & \multicolumn{2}{c|}{$m=128$} & \multicolumn{2}{c|}{$m=256$} & \multicolumn{2}{c}{$m=512$} \\  
 & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & $\Delta$\textit{perf} ($\downarrow$) \\
 \midrule 
 \multicolumn{9}{l}{\it {Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
\midrule
 SGD  & 191.61\std{13.75} & 101.56\std{9.22} & 191.61\std{13.75} & 101.56\std{9.22} & 191.61\std{13.75} & 101.56\std{9.22} & 191.61\std{13.75} & 101.56\std{9.22} \\
 A-GEM   &  43.61\std{0.74} & 48.00\std{0.94} & 44.10\std{2.31} & 50.20\std{2.76} & 38.88\std{1.85} & 49.01\std{2.88} & 24.88\std{3.14} & 50.85\std{4.68} \\
 ER     &  40.18\std{1.85} & 20.70\std{0.47} & 24.67\std{1.38} & 13.82\std{0.70} & 14.73\std{3.06} & 8.52\std{0.46} & 8.27\std{0.80} &  5.44\std{2.44} \\
\bf CAR &   13.37\std{3.64} & 23.25\std{2.81} & 6.25\std{0.72} & 19.32\std{3.05} & 4.29\std{0.24} & 12.43\std{3.80} &  2.18\std{0.80} & 10.80\std{2.19} \\
 \midrule
 \multicolumn{9}{l}{\it {Sequence}: \textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
\midrule
 SGD  & 110.48\std{16.28} & 79.45\std{14.32} & 110.48\std{16.28} & 79.45\std{14.32} & 110.48\std{16.28} & 79.45\std{14.32} & 110.48\std{16.28} & 79.45\std{14.32} \\
 A-GEM   &  46.52\std{4.31} & 63.99\std{4.85} & 48.94\std{2.98} & 62.27\std{3.97} & 46.71\std{4.81} & 71.69\std{4.89} & 32.55\std{5.12} & 60.06\std{5.65} \\
 ER  &  43.75\std{2.70} & 33.42\std{3.20} & 24.00\std{4.46} & 24.29\std{3.20} & 19.86\std{6.44} & 12.65\std{4.48} & 9.14\std{3.92} &  5.27\std{2.88} \\
\bf CAR & 15.92\std{4.59} & 35.60\std{3.09} & 7.86\std{2.55} & 26.77\std{4.48} & 6.71\std{1.24} & 14.31\std{0.73} & 5.69\std{3.05} & 10.76\std{1.14} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{center}
\end{table*}
\fi

==> compressed activation replay ICLR 2021/tables/taskonomy_buffer_filling.tex <==
\begin{table*}
\caption{\textbf{Buffer filling techniques (taskonomy):}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $3$ random seeds.}
\label{tab:taskonomy_buffer_filling}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
 & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) \\
 \midrule 
 \multicolumn{9}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
\midrule
 Reservoir Sampling & 31.43 & 17.59 & 21.51 & 15.06 & 13.93 & 9.29 & 5.67 & 5.65 \\
 Hard Example Mining & 45.28 & 53.90 & 43.64 & 48.87 & 35.70 & 37.02 & 28.02 & 24.59 \\
 Easy Example Mining & 62.91 & 46.21 & 54.96 & 46.20 & 43.50 & 36.54 & 35.32 & 33.53 \\
 High Variance Filling & 37.46 & 26.43 & 23.51 & 18.13 & 16.02 & 9.95 & 3.05 & 7.32 \\
 Loss Equilization & 32.99 & 20.82 & 24.41 & 13.88 & 12.50 & 8.29 & 6.29 & 4.70 \\
 Loss Equilization (importance) & 31.12 & 17.91 & 22.94 & 12.00 & 13.78 & 8.36 & 9.08 & 5.50 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

%  Reservoir Sampling & 31.43 & 17.59 & 21.51 & 15.06 & 13.93 & 9.29 & 5.67 & 5.65 \\
%  Reservoir Sampling & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\

==> compressed activation replay ICLR 2021/tables/taskonomy_compression.tex <==
\begin{table*}
\caption{\small \textbf{Taskonomy compression techniques:} Forgetting (\textit{fgt}), performance drop ($\Delta$\textit{perf}) and memory overhead (\textit{mem}) values are reported. All results are averaged over $3$ random seeds.}
\vskip -1em
\label{tab:taskonomy_compression}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|ccc|ccc|ccc|ccc}
\toprule
Compression & \multicolumn{3}{|c}{$m=64$}  & \multicolumn{3}{|c}{$m=128$} & \multicolumn{3}{|c}{$m=256$} & \multicolumn{3}{|c}{$m=512$} \\  
 Method& \textit{fgt} & $\Delta$\textit{perf} & \textit{mem} & \textit{fgt} & $\Delta$\textit{perf}  & \textit{mem} & \textit{fgt} & $\Delta$\textit{perf} & \textit{mem} & \textit{fgt}  & $\Delta$\textit{perf} &  \textit{mem} \\
 \midrule 
 \midrule
 No compression  & 9.18 & 29.45 & 335.5M & 4.33 & 22.73 & 671.0 M & 0.77 & 22.06 & 1.3 G & 0.51  & 15.44 & 2.7 G \\
 \midrule
 Spatial & 18.15 & 31.45 & 5.1 M & 9.78 & 23.58 & 10.2 M & 7.75 & 16.31 & 20.4 M & 4.30 & 12.53 & 41.0 M \\
 Channel & 18.00 & 18.25 & 0.2 M & 21.38 & 33.22 & 0.3 M & 6.83  & 28.40 & 0.6 M & 6.47 & 28.28 & 1.3 M \\
 Spatial + Channel   & 12.43 & 25.97 & 5.4 M & 6.25  & 19.32 & 10.8 M & 4.29 & 15.62 & 21.6 M & 2.18 & 10.80 & 43.3 M \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{center}
\end{table*}

==> compressed activation replay ICLR 2021/tables/taskonomy_deprecated.tex <==
% \begin{table*}
% \caption{\textbf{Taskonomy Results:} Continual learning performance of various techniques  -- \textit{E}: Expansion based, \textit{R}: Regularization based and $M$: memory based. Forgetting (\textit{fgt}) and oracle performance drop (\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
% \label{tab:taskonomy}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l |c|cc|cc|cc|cc}
% \toprule
% Method & Type & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
%  & & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) \\
%  \midrule 
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
% \midrule
%  Vanilla SGD  & & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 \\
%  EWC & \textit{R} & &  &  &  &  &  \\
%  AGEM   & \textit{M} & 43.61 & 48.00 & 44.10 & 50.20 & 38.88 & 49.01 & 24.88 & 50.85 \\
%  ER     & \textit{M} & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\
%  CAER (ours) & \textit{M}  & 13.37 & 23.25 & 4.80 & 17.32 & 2.98 & 12.43 & 1.91 & 11.51 \\
%  \midrule
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
% \midrule
%  Vanilla SGD  & & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 \\
%  EWC & \textit{R} &  &  &  &  &  \\
%  AGEM   & \textit{M} & 46.52 & 63.99 & 48.94 & 62.27 & 46.71 & 71.69 & 32.55 & 60.06 \\
%  ER  & \textit{M}   & 43.75 & 33.42 & 24.00 & 24.29 & 19.86 & 12.65 & 9.14 & 5.27 \\
%  CAER (ours) & \textit{M}  & 15.92 & 35.60 & 7.86 & 26.77 & 6.71 & 14.31 & 5.69 & 10.76 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}


==> compressed activation replay ICLR 2021/tables/taskonomy_experiment_details.tex <==
\begin{table*}
\caption{\textbf{Experiment details on Taskonomy dataset}}
\label{tab:exp_details_taskonomy}
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l}
\toprule
    Encoder Architecture    & Resnet-50 \\
    Decoder Architecture    & 15-layer ConvNet for pixelwise tasks \\
                            & Average pooling + 1 FC layer for classification \\
    Encoder Learning rate   & 0.0001    \\
    Decoder Learning rate   & 0.0001    \\
    Optimizer               & Adam      \\
    LR Decay                & None      \\
    Batch Size              & 64        \\
    Effective number of training iters    & 12500 per task    \\
    
    \midrule
    \multicolumn{2}{c}{Experience Replay} \\
    \midrule
    Buffer filling strategy & Uniform Sampling \\
    Replay batch size       & 64 \\
    Replay probability $p_{replay}$     & 0.5 \\
    
    \midrule
    \multicolumn{2}{c}{CAR} \\
    \midrule
    Regularization function $\ell_{fm}$ & MSE loss \\
    Compression scheme      & Spatial + channel pooling \\
    Replay probability $p_{replay}$     & 0.5 \\
    
    \midrule
    \multicolumn{2}{c}{Side Tuning} \\
    \midrule
    Side Network Architecture   & 5-layer ConvNet   \\
    Side Network Learning rate  & 0.0001 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> compressed activation replay ICLR 2021/tables/taskonomy_no_car.tex <==
% \begin{table*}
% \caption{\textbf{Taskonomy Results:} Continual learning performance of various techniques  -- \textit{E}: Expansion based, \textit{R}: Regularization based and $M$: memory based. Forgetting (\textit{fgt}) and oracle performance drop (\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
% \label{tab:taskonomy}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l |c|cc|cc|cc|cc}
% \toprule
% Method & Type & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
%  & & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) \\
%  \midrule 
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
% \midrule
%  Vanilla SGD  & & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 \\
%  Side-Tuning$^*$ & \textit{E} & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 \\
%  EWC & \textit{R} & &  &  &  &  &  \\
%  AGEM   & \textit{M} & 43.61 & 48.00 & 44.10 & 50.20 & 38.88 & 49.01 & 24.88 & 50.85 \\
%  ER     & \textit{M} & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\
%  \midrule
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
% \midrule
%  Vanilla SGD  & & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 \\
%  EWC & \textit{R} &  &  &  &  &  \\
%  AGEM   & \textit{M} & 46.52 & 63.99 & 48.94 & 62.27 & 46.71 & 71.69 & 32.55 & 60.06 \\
%  ER  & \textit{M}   & 43.75 & 33.42 & 24.00 & 24.29 & 19.86 & 12.65 & 9.14 & 5.27 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}


==> figures/tsne_CAER.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/TSNE_plot_FM.png}
\caption{\textbf{Visualizing t-SNE embeddings} of model trained using Compressed Activation Replay on Split-CIFAR dataset. We compare the features of the encoder of the final model (\emph{shown in blue}) relative to the encoder representations obtained while training the respective tasks (\emph{shown in red}). Feature space drift on older tasks are significantly reduced compared to experience replay (Figure~\ref{fig:tsne_ER}). }
\label{fig:tsne_CAER} 
\end{figure*}

==> replay_buffer_strategies.tex <==

\section{Replay Buffer Filling Strategies}

\input{tables/taskonomy_buffer_filling.tex}

One of the components of experience replay pipeline is the strategy to fill the replay buffer. The replay buffer $\cM$ can store $m$ samples per task. In this section, we investigate several strategies for filling the buffer. While some of the recent papers have proposed strategies for classification tasks, they cannot be extended for regression problems. Our objective is to study buffer filling strategies for any generic loss function. We investigate the following strategies:

\textit{1. Reservoir sampling}: This is the most commonly used strategy in experience replay pipelines. The idea is to fill the replay buffer uniformly at random from the data sequence seen thus far.

\textit{2. Hard example mining}: In this technique, we fill the replay buffer with samples having the maximum training loss as they may capture the decision boundaries well.

\textit{3. Easy example mining}: Here, we fill the replay buffer with samples having the minimum training loss with the hope that easy samples are typical representatives of the tasks.

\textit{4. High variance filling}: The idea is to store samples having large running variance over the course of training the respective task. During training, we update running variance of training samples for the respective task, and store samples that have high running variance in the replay buffer.

\textit{5. Loss equalization}: In this technique, we maintain and update the loss histogram of each task during training. We then store samples at uniform interval from this histogram. This results in having a flat loss histogram in the replay buffer.

\textit{6. Loss equalization with importance weighting}: In the loss equalization technique, the loss distribution of samples in the replay buffer is different from the original task loss distribution. To prevent this issue, we store sample weights which are proportional to the height of the loss histogram in the replay buffer. While sampling from the buffer, we use these weights as sampling probabilities.


\input{tables/split_cls_buffer_filling.tex}

\paragraph{Discussion: } The results of storing samples using these buffer filling strategies are shown in Table.~\ref{tab:taskonomy_buffer_filling}. The standard Reservoir Sampling shows strong performance among all sampling strategies. One promising strategy is loss equalization, which outperforms reservoir sampling in the Taskonomy dataset. Table~\ref{tab:split_cls_buffer_filling} shows the same comparative experiment on Split-CIFAR and Split-MiniImageNet. In this table, we observe that Reservoir Sampling is also very competitive. Loss equalization does not show any advantage over reservoir sampling in these two datasets. However, easy example mining marginally improves both accuracy and forgetting metrics over the standard reservoir sampling strategy.

As we can tell from the two tables, there is no single replay methods that outperform the rest in all three datasets. One potential reason is that the Taskonomy dataset contains different kinds of tasks including classification and regression while CIFAR and Mini-Imagenet are both classification datasets. More complex tasks may need different behaviours for the approaches. The results also suggest that the current benchmark for continual learning may not be sufficient to study and evaluate the effectiveness of different approaches. 
These findings cal for developer yet larger scale benchmark that can further challenge the existing methodologies that can really boost the continual learning performance. As a takeaway from this experiment, the standard reservoir sampling seems to be a competitive approach on different dataset conditions, perhaps because it was developed with minimum assumptions on the data distributions. Further theoretical study of this phenomena remains as an interesting future direction. 


==> tables/split_cifar.tex <==
\begin{table*}
\caption{\textbf{Split-CIFAR Results:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cifar}
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=255$} & \multicolumn{2}{|c}{$m=425$} \\  
 & Accuracy & Forgetting & Accuracy  & Forgetting & Accuracy & Forgetting \\
 \midrule \midrule 
 EWC    & 42.4 & 0.25 & - & - & - & - \\


 ICARL  & 46.4 & 0.16 & 51.7 & 0.13 & 51.2 & 0.13 \\
 AGEM   & 54.9 & 0.14 & 56.9 & 0.13 & 59.9 & 0.10 \\
 MER    & 49.7 & 0.19 & 57.7 & 0.11 & 60.6 & 0.09 \\
 ER     & 56.2 & 0.13 & 60.9 & 0.09 & 62.6 & 0.06 \\
 HAL    & 60.4 & 0.10 & 62.9 & 0.08 & 64.4 & 0.06 \\
 \midrule
 CAR (ours)  & 62.4 &  0.06 & 65.2 &  0.05 & 66.5 &  0.04 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> tables/split_cls_buffer_filling.tex <==
\begin{table*}
\caption{\textbf{Buffer filling techniques:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_cls_buffer_filling}
\begin{center}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|cc|cc  ||  cc|cc}
\toprule
 & \multicolumn{4}{|c||}{Split-CIFAR} & \multicolumn{4}{|c}{Split-miniImagenet} \\  
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c||}{$m=425$} & \multicolumn{2}{|c}{$m=85$} & \multicolumn{2}{|c}{$m=425$} \\  
 & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} & \textit{acc} & \textit{fgt} \\
\midrule
 Reservoir Sampling & 56.1 & 0.12 & 63.4 & 0.07 & 50.0 & 0.09 & 53.2 & 0.08 \\
 Hard Example Mining & 45.1 & 0.22 & 55.0 & 0.14 & 39.4 & 0.18 & 45.4 & 0.14 \\
 Easy Example Mining & 56.6 & 0.09 & 64.1 & 0.06 & 50.0 & 0.08 & 55.4 & 0.06 \\
 High Variance Filling & 56.4 & 0.12 & 63.7 & 0.07 & 50.6 & 0.08 & 52.6 & 0.09 \\
 Loss Equilization & 49.6 & 0.19 & 61.4 & 0.09 & 45.6 & 0.13 & 53.0 & 0.08 \\
 Loss Equilization (importance) & 52.1 & 0.16 & 61.6 & 0.08 & 45.4 & 0.13 & 52.2 & 0.09 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> tables/split_imagenet.tex <==
\begin{table*}
\caption{\textbf{Split-miniImagenet Results:}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $5$ random seeds.}
\label{tab:split_miniimagenet}
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=85$}  & \multicolumn{2}{|c|}{$m=255$} & \multicolumn{2}{|c}{$m=425$} \\  
 & Accuracy & Forgetting & Accuracy  & Forgetting & Accuracy & Forgetting \\
 \midrule \midrule 
 EWC    & 37.7 & 0.21 & - & - & - & - \\


 AGEM   & 48.2 & 0.13 & 51.6 & 0.10 & 54.3 & 0.08 \\
 MER    & 45.5 & 0.15 & 49.4 & 0.12 & 54.8 & 0.07 \\
 ER     & 49.0 & 0.12 & 53.5 & 0.07 & 54.2 & 0.08 \\
 HAL    & 51.6 & 0.10 &  56.5 &  0.06 &  57.2 &  0.06 \\
 \midrule
 CAR (ours)  &  54.2 &  0.06 & 55.1 &  0.06 & 56.2 &  0.06 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> tables/taskonomy_buffer_filling.tex <==
\begin{table*}
\caption{\textbf{Buffer filling techniques (taskonomy):}  Accuracy $(in \%)$ and forgetting values are reported. All results are averaged over $3$ random seeds.}
\label{tab:taskonomy_buffer_filling}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
Method & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
 & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) & Fgt ($\downarrow$) & Perf ($\downarrow$) \\
 \midrule 
 \multicolumn{9}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
\midrule
 Reservoir Sampling & 31.43 & 17.59 & 21.51 & 15.06 & 13.93 & 9.29 & 5.67 & 5.65 \\
 Hard Example Mining & 45.28 & 53.90 & 43.64 & 48.87 & 35.70 & 37.02 & 28.02 & 24.59 \\
 Easy Example Mining & 62.91 & 46.21 & 54.96 & 46.20 & 43.50 & 36.54 & 35.32 & 33.53 \\
 High Variance Filling & 37.46 & 26.43 & 23.51 & 18.13 & 16.02 & 9.95 & 3.05 & 7.32 \\
 Loss Equilization & 32.99 & 20.82 & 24.41 & 13.88 & 12.50 & 8.29 & 6.29 & 4.70 \\
 Loss Equilization (importance) & 31.12 & 17.91 & 22.94 & 12.00 & 13.78 & 8.36 & 9.08 & 5.50 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

%  Reservoir Sampling & 31.43 & 17.59 & 21.51 & 15.06 & 13.93 & 9.29 & 5.67 & 5.65 \\
%  Reservoir Sampling & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\

==> tables/taskonomy_deprecated.tex <==
% \begin{table*}
% \caption{\textbf{Taskonomy Results:} Continual learning performance of various techniques  -- \textit{E}: Expansion based, \textit{R}: Regularization based and $M$: memory based. Forgetting (\textit{fgt}) and oracle performance drop (\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
% \label{tab:taskonomy}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l |c|cc|cc|cc|cc}
% \toprule
% Method & Type & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
%  & & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) \\
%  \midrule 
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
% \midrule
%  Vanilla SGD  & & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 \\
%  EWC & \textit{R} & &  &  &  &  &  \\
%  AGEM   & \textit{M} & 43.61 & 48.00 & 44.10 & 50.20 & 38.88 & 49.01 & 24.88 & 50.85 \\
%  ER     & \textit{M} & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\
%  CAER (ours) & \textit{M}  & 13.37 & 23.25 & 4.80 & 17.32 & 2.98 & 12.43 & 1.91 & 11.51 \\
%  \midrule
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
% \midrule
%  Vanilla SGD  & & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 \\
%  EWC & \textit{R} &  &  &  &  &  \\
%  AGEM   & \textit{M} & 46.52 & 63.99 & 48.94 & 62.27 & 46.71 & 71.69 & 32.55 & 60.06 \\
%  ER  & \textit{M}   & 43.75 & 33.42 & 24.00 & 24.29 & 19.86 & 12.65 & 9.14 & 5.27 \\
%  CAER (ours) & \textit{M}  & 15.92 & 35.60 & 7.86 & 26.77 & 6.71 & 14.31 & 5.69 & 10.76 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}


==> tables/taskonomy_no_car.tex <==
% \begin{table*}
% \caption{\textbf{Taskonomy Results:} Continual learning performance of various techniques  -- \textit{E}: Expansion based, \textit{R}: Regularization based and $M$: memory based. Forgetting (\textit{fgt}) and oracle performance drop (\textit{perf}) values are reported. All results are averaged over $3$ random seeds.}
% \label{tab:taskonomy}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l |c|cc|cc|cc|cc}
% \toprule
% Method & Type & \multicolumn{2}{|c|}{$m=64$}  & \multicolumn{2}{|c|}{$m=128$} & \multicolumn{2}{|c}{$m=256$} & \multicolumn{2}{|c}{$m=512$} \\  
%  & & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) & \textit{fgt} ($\downarrow$) & \textit{perf} ($\downarrow$) \\
%  \midrule 
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Curv, Cls (obj), Normal, Seg, Depth, Reshade, Edge (tex), Cls (sc), Keypts2d, Edge (occ), Keypts3d}} \\
% \midrule
%  Vanilla SGD  & & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 & 191.61 & 101.56 \\
%  Side-Tuning$^*$ & \textit{E} & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 & 0.0 & 53.99 \\
%  EWC & \textit{R} & &  &  &  &  &  \\
%  AGEM   & \textit{M} & 43.61 & 48.00 & 44.10 & 50.20 & 38.88 & 49.01 & 24.88 & 50.85 \\
%  ER     & \textit{M} & 40.18 & 20.70 & 24.67 & 13.82 & 14.73 & 8.52 & 8.27 & 5.44 \\
%  \midrule
%  \midrule
%  \multicolumn{10}{c}{\textbf{Sequence}: \textit{Depth, Keypts2d, Seg, Normal, Cls (obj), Curv, Edge (occ), Reshade, Cls (sc), Keypts3d, Edge (tex)}} \\
% \midrule
%  Vanilla SGD  & & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 & 110.48 & 79.45 \\
%  SideTuning$^*$ & \textit{E} & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 & 0.0 & 29.97 \\
%  EWC & \textit{R} &  &  &  &  &  \\
%  AGEM   & \textit{M} & 46.52 & 63.99 & 48.94 & 62.27 & 46.71 & 71.69 & 32.55 & 60.06 \\
%  ER  & \textit{M}   & 43.75 & 33.42 & 24.00 & 24.29 & 19.86 & 12.65 & 9.14 & 5.27 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}

